Network Structure Inference, A Survey: Motivations, Methods, and Applications

Networks represent relationships between entities in many complex systems, spanning from online social interactions to biological cell development and brain connectivity. In many cases, relationships between entities are unambiguously known: are two users 'friends' in a social network? Do two researchers collaborate on a published paper? Do two road segments in a transportation system intersect? These are directly observable in the system in question. In most cases, relationship between nodes are not directly observable and must be inferred: does one gene regulate the expression of another? Do two animals who physically co-locate have a social bond? Who infected whom in a disease outbreak in a population? Existing approaches for inferring networks from data are found across many application domains and use specialized knowledge to infer and measure the quality of inferred network for a specific task or hypothesis. However, current research lacks a rigorous methodology which employs standard statistical validation on inferred models. In this survey, we examine (1) how network representations are constructed from underlying data, (2) the variety of questions and tasks on these representations over several domains, and (3) validation strategies for measuring the inferred network's capability of answering questions on the system of interest.

==> applications-ppi.tex <==
PPI: \cite{Stelzl2005957, Liu2009, 20158874, Sharan2007}

\cite{DeJuan2013, Csermely2013}

==> backup.tex <==
\subsection{Formulating Data-to-Task Workflows with Network Data Models}

Our problem definition is flexible enough to incorporate the varying types of network models (\emph{e.g.,} regression, parametric network models) and tasks (\emph{e.g.,} prediction, descriptive statistics and hypothesis testing). Below, we describe several formulations for network structure inference, according to their network model and task model. 

\subsubsection{Interaction Networks}
\label{subsubsec:interaction}

The most prevalent class of network topology inference is measuring pairwise interactions (\emph{e.g.,} correlations) between nodes, and choosing a threshold to define a sufficient degree of interaction. This threshold may be chosen by some statistical test, by tuning on some desired criteria (\emph{e.g.,} assumed network density), or in an ad-hoc way with prior domain knowledge.

This has been discussed in the context of \emph{discrete} interactions as described above: 

\begin{displayquote}
``Inferring networks from pairwise interactions of cell-phone call or email records simply reduces down to selecting the right threshold $\tau$ such that an edge (u, v) is included in the network if u and v interacted more than $\tau$ times in the dataset. Similarly, inferring networks of interactions between proteins in a cell usually reduces to determining the right threshold.'' \cite{NIPS2010_4113}
\end{displayquote}

%\blockquote{We discretize by setting a threshold to the ratio between measured expression and control. In our experiments we choose a threshold value of 0.5 in logarithmic (base 2) scale\cite{Friedman00usingbayesian}}

Researchers often make several application-specific decisions around these thresholds:

\begin{displayquote}
``From this complete correlation graph, only the edges with significant correlation ($>0.5$) were retained. But using the same threshold for positive and negative correlations is not appropriate as negative correlations are usually weaker and many nearby locations have high positive correlation'' \cite{Kawale2013}
\end{displayquote}

\begin{displayquote}
``We let $\delta$ as a user-controlled parameter, where larger $\delta$ values correspond to less predicted regulations, and only focus on designing a significance score s(t,g) that leads to `good' prediction for some values of $\delta$'' \cite{23173819}
\end{displayquote}

These methods typically produce a fixed network model but do not explore the space of possible networks under varying interaction thresholds, except through offline trial-and-error. Furthermore, subsequent sensitivity analysis on these outputted networks $G$ are often performed on the task model parameters alone, rather than jointly on both models.

We can formulate the workflow for this analysis under our framework. Assume the interaction threshold $\tau$ is given by hand-tuning or domain knowledge, we have some feature matrix $\mathbf{D}$ that has some notion of similarity between features, and $\mathcal{T}()$ is an edge prediction task evaluated on $\mathbf{E}^*$. Then this workflow is expressed as: 

\begin{equation} 
	\label{eq:simple_th} 
	\mathcal{R}(\mathbf{D}, \mathbf{\tau}) \rightarrow \mathbf{G}; \argmin_{\mathbf{\beta}} e(\mathcal{T}(\mathbf{G}, \mathbf{\beta}), \mathbf{E}^*)
\end{equation}

When these interaction networks are evaluated in the absence of ground truth, the network may be measured through autocorrelation. In this case, the same network inference is applied, $\mathcal{R}(\mathbf{D^*}, \mathbf{\alpha})  \rightarrow \mathbf{G^*}$ for some hold-out data $D^*$ (\emph{e.g.,} at some later time).

\subsubsection{Parametric Inference and Model-Fit Networks}

Maximum-likelihood methods assume some parametric model family to represent relationships between nodes (such as time between interaction, likelihood of information transmission over time) and infer the best model parameters. For clarity, we work through one specific application, in epidemiology and information networks such as blogs, although the pattern is similar in other applications. Structure inference methods on information networks share the assumption that we are observing the `arrival' of information or attribute value at nodes (\emph{i.e.,} computers, blog pages, individuals) over time, but are unable to observe the topology which transmitted the information. For an edge $e_{ij}$, the infection time difference $t_j - t_i$ can be fit against an infection model over time, measuring the likelihood that $v_i$ infected $v_j$ \cite{NIPS2010_4113}.

Where input data $\mathbf{D}$ are infection times of each node, we can formulate these workflows as:
\begin{equation} 
	\label{eq:maximum_likelihood} 
	\argmin_{\mathbf{\alpha}} \mathcal{R}(\mathbf{D}, \mathbf{\alpha}) \rightarrow \mathbf{G};  \argmin_{\mathbf{\beta}} e(\mathcal{T}(\mathbf{G}, \mathbf{\beta}), \mathbf{E}^*)
\end{equation}

In information network applications, $\mathbf{E}^*$ is typically provided by a known network. Processes are simulated on this network to generate input data for the maximum-likelihood relational data model $\mathcal{R}()$. This method is used to `reconstruct' $\mathbf{E}^*$ only from input data $\mathbf{D}$. 

\subsubsection{Jointly-Learned Network and Task Models}
\label{subsubsec:joint}
Previous work in statistical relational learning on \emph{explicit} networks has focused on jointly learning relationships between (categorical) attributes and a predictive task, such as link prediction \cite{Gong:2014:JLP:2611448.2594455,namata:tkdd15}, and distinguishing correlated effects between these processes \cite{LaFond:2010:RTD:1772690.1772752}. 

Previous work has also used a \emph{workflow} approach to the network structure inference problem which maximizes performance of particular task(s) on the inferred network \cite{DeChoudhury:2010:IRS:1772690.1772722, Farine2016}. Consider interaction networks over varying thresholds $\tau$. A naive solution for this type of approach is to explore the parameter space of $\mathcal{R}(\mathbf{D}, \tau)$ and evaluate the task performance on each inferred network. However, this is very costly, especially as $\mathcal{R}$ requires more parameters. 

The joint optimization for network structure inference learns the features in $\mathbf{D}$ that perform well at task $\mathcal{T}()$. For example, previous work has learned network models which jointly discovers features in a supervised LDA model, and the logistic regression weights which perform well for an edge prediction task \cite{McAuley:2015:INS:2783258.2783381}. In Equation \ref{eq:joint_opt}, we have already formulated joint optimization network structure inference within our framework, repeated here:
\begin{equation} 
	\label{eq:joint_opt2} 
	\argmin_{\mathbf{G}} e(\mathcal{T}(\mathcal{R}(\mathbf{D}, \mathbf{\alpha}), \mathbf{\beta}), \mathbf{E}^*)
\end{equation}

The jointly optimized model may avoid discovering spurious relational model parameters which are not suitable for the intended task. Second, we may be able to learn a more interpretable relationship between the original feature space and the task model. However, this strategy has the added requirement that the output of each model can be used to re-train the other. For example, \citet{McAuley:2015:INS:2783258.2783381} use a \emph{supervised} LDA model which uses the output of the edge prediction task to re-train the relational model. Because of this added modeling complexity, joint models are relatively rare compared with multi-step workflows.


==> backup_new.tex <==



\section{A Taxonomy for Network Structure Inference}
\label{sec:problem}

\subsection{Data Science Motivations for Network Structure Inference}

Data science has been a growing and quickly-evolving field of study in recent years. Under the name `Data-intensive science,' Jim Gray argues that data and computation enable a new `fourth' paradigm of science. These data-driven models enable the investigation of questions beyond the \emph{capability} of science utilizing theoretical model-driven (the second) or model-driven simulation (the third) paradigms \cite{Hey2009}. We organize the network inference problem through a lens of hypothesis-driven data science. Under this perspective, the value of a network can be stated simply: for a scientific question of interest, and its relevant (non-network) data, are networks an informative and useful \emph{data model} for \emph{better} answering our question?

\begin{figure}
\centering{\includegraphics[width=1\columnwidth]{figs/datascience}}
\caption{A general framework for computational science and data science, with a focus on networks as data models for non-network data. A researcher typically (1) uses \emph{relevant} data and \emph{appropriate} data models to formalize a particular question. Traditional domain science (top, orange) typically combines direct observation and simple statistical models. Data-driven science with machine learning (bottom, purple) augments this intuition, hypotheses and statistical models with sophisticated features and patterns, yielding additional challenges for visualization, hypothesis testing and generation. The output of this analysis is a plausible explanation or some supported hypothesis. The result of data-driven science are considered to be shrinking this `gap' in understanding, toward robust and verifiable answers to the original question, in novel ways (see: \cite{Hey2009}).}
\label{fig:datascience}
\end{figure}

Figure \ref{fig:datascience} gives an overview of this data science workflow, and all the relevant terms to our taxonomy. As researchers, we start with a broad question of interest, and try to locate or collect the data relevant to answering our question. There are several possible data sources and modalities for analysis, coupled with several possible representations (including networks). Our choice of data representation informs and constrains our hypotheses about the question of interest, and typically domain science (orange, top) and machine learning (purple, bottom) generate complimentary results for hypothesis generation and testing. Novel computational models are developed to test these hypotheses. Results from this data-driven paradigm have closed the gap in understanding for many questions in novel ways. Data-driven science has also developed novel methodologies, enabling new, large-scale experimental design \cite{Gui:2015:NAT:2736277.2741081,Backstrom:2011:NBT:1963405.1963492} and randomization techniques \cite{efron93bootstrap, RSSB:RSSB12050}, two key methodologies across scientific domains. 

Figure \ref{fig:datascience} highlights several levels of modeling which can impact the final performance at answering our question of interest. Often different individuals will be responsible for generating or collecting the underlying data, inferring or defining the network, and developing the predictive models. For example, machine learning researchers will rarely control the underlying sampling rate of very specialized data collection workflows in bioinformatics, geophysics and climate, or neuroscience. In the machine learning community, there is a great deal of sensitivity analysis for the subsequent predictive method parameters, without testing the parameters of the underlying network representation. This strategy is effective at producing sophisticated models ``given a network,'' but is less suited at answering our scientific questions on the original data or system.

% \subsection{Taxonomy}
% \label{subsec:taxonomy}

\subsubsection{Taxonomy}

We taxonomize work in the network inference problem according to (1) the varying `difficulty' of defining edges and nodes given the nature of the \emph{underlying data} of the network, (2) the types of \emph{questions} and hypotheses which are studied using the network representation (3) the \emph{type of method} (e.g. regression, correlation, novel interaction measures) used for inference. 

\subsection{Defining Edges and Nodes}

\subsubsection{Explicit, Discrete, and Inferred Edge Definitions}

Networks model three broad types of relationships (\emph{i.e.,} edges), typically based on a measure of interaction between entities. Categorical, \emph{explicit} relationships are unambiguously known in the system--such as the `friend' relation in Facebook. \emph{Discrete} interactions denote unambiguous transactions occurring between two entities--such as phone calls or text messages in mobile device data. The primary task of defining edges on these interactions is to select an appropriate threshold to measure the strength of the relationship. \emph{Inferred} interactions denote some statistical measure of similarity, beyond simple transaction counts. For example, the definition of a spatiotemporal \emph{co-location} interaction between two entities can be simply inferred by specifying ``how close'' for ``what duration.'' This is generally a more challenging measure of relationships relative to discrete interactions.

\subsubsection{Explicit and Inferred Node Definitions}

Similarly, inferring nodes is of varying difficulty in different domains. In most applications, the nodes are explicit in two ways: (1) the node definition is unambiguous (e.g. a `user', `individual' or `gene' is a node), and (2) there is a node \emph{correspondence} between time-steps in the data (e.g. this particular node corresponds to user `i' at each time step). Functional brain networks, and climate networks are two examples of domains where the node definition is not explicitly given--e.g. a group of two-dimensional earth surface pixels, or three-dimensional brain voxels. The \emph{scale} of node definition can dramatically change the performance of predictive models, or the stability of descriptive statistics derived from the network \cite{Cammoun2012386}.


\subsection{Types of Network Models}

A network model defines or learns the above edge/node definitions based on rule-based criteria, some statistical model on underlying data, or task-based validation against some objective of interest. 

\subsubsection{Interaction Networks}
\label{subsubsec:interaction}

The most prevalent class of network topology inference is measuring pairwise interactions (e.g. correlations) between nodes, and choosing a threshold to define a sufficient degree of interaction. This threshold may be chosen by some statistical test, by tuning on some desired criteria (e.g. assumed network density), or in an ad-hoc way with prior domain knowledge.

This has been discussed in the context of \emph{discrete} interactions as described above: 

\begin{displayquote}
``Inferring networks from pairwise interactions of cell-phone call or email records simply reduces down to selecting the right threshold $\tau$ such that an edge (u, v) is included in the network if u and v interacted more than $\tau$ times in the dataset. Similarly, inferring networks of interactions between proteins in a cell usually reduces to determining the right threshold.'' \cite{NIPS2010_4113}
\end{displayquote}

%\blockquote{We discretize by setting a threshold to the ratio between measured expression and control. In our experiments we choose a threshold value of 0.5 in logarithmic (base 2) scale\cite{Friedman00usingbayesian}}

Researchers often make several application-specific decisions around these thresholds:

\begin{displayquote}
``From this complete correlation graph, only the edges with significant correlation ($>0.5$) were retained. But using the same threshold for positive and negative correlations is not appropriate as negative correlations are usually weaker and many nearby locations have high positive correlation'' \cite{Kawale2013}
\end{displayquote}

\begin{displayquote}
``We let $\delta$ as a user-controlled parameter, where larger $\delta$ values correspond to less predicted regulations, and only focus on designing a significance score s(t,g) that leads to `good' prediction for some values of $\delta$'' \cite{23173819}
\end{displayquote}

These methods typically produce a fixed network model but do not explore the space of possible networks under varying interaction thresholds, except through offline trial-and-error. Furthermore, subsequent sensitivity analysis on these outputted networks $G$ are often performed on the task model parameters alone, rather than jointly on both models.

We can formulate the workflow for this analysis under our framework. Assume the interaction threshold $\tau$ is given by hand-tuning or domain knowledge, we have some feature matrix $\mathbf{D}$ that has some notion of similarity between features, and $\mathcal{T}()$ is an edge prediction task evaluated on $\mathbf{E}^*$. Then this workflow is expressed as: 

\begin{equation} 
	\label{eq:simple_th} 
	\mathcal{R}(\mathbf{D}, \mathbf{\tau}) \rightarrow \mathbf{G}; \argmin_{\mathbf{\beta}}~ e(\mathcal{T}(\mathbf{G}, \mathbf{\beta}), \mathbf{E}^*)
\end{equation}

When these interaction networks are evaluated in the absence of ground truth, the network may be measured through autocorrelation. In this case, the same network inference is applied, $\mathcal{R}(\mathbf{D^*}, \mathbf{\alpha})  \rightarrow \mathbf{G^*}$ for some hold-out data $D^*$ (e.g. at some later time).

\subsubsection{Parametric Inference and Model-Fit Networks}

Maximum-likelihood methods assume some parametric model to represent relationships between nodes (such as time between interaction, likelihood of information transmission over time) and infer the best model parameters. For clarity, we work through one specific application, in epidemiology and information networks such as blogs, although the pattern is similar in other applications. Structure inference methods on information networks share the assumption that we observe the `arrival' of information or attribute value at nodes (\emph{i.e.,} computers, blog pages, individuals) over time, but are unable to observe the topology which transmitted the information. For an edge $e_{ij}$, the infection time difference $t_j - t_i$ can be fit against an infection model over time, measuring the likelihood that $v_i$ infected $v_j$ \cite{NIPS2010_4113}.

% Where input data $\mathbf{D}$ are infection times of each node, we can formulate these workflows as:
% \begin{equation} 
% 	\label{eq:maximum_likelihood} 
% 	\argmin_{\mathbf{\alpha}} \mathcal{R}(\mathbf{D}, \mathbf{\alpha}) \rightarrow \mathbf{G};  \argmin_{\mathbf{\beta}} e(\mathcal{T}(\mathbf{G}, \mathbf{\beta}), \mathbf{E}^*)
% \end{equation}

In information network applications, validation data is typically provided by a known network. Processes are simulated on this network to generate input data for the maximum-likelihood network model parameters. This method is used to `reconstruct' the ground truth network only from simulated input data. 

\subsubsection{Jointly-Learned Network and Task Models}
\label{subsubsec:joint}
Previous work in statistical relational learning on \emph{explicit} networks has focused on jointly learning relationships between (categorical) attributes and a predictive task, such as link prediction \cite{Gong:2014:JLP:2611448.2594455,namata:tkdd15}, and distinguishing correlated effects between these processes \cite{LaFond:2010:RTD:1772690.1772752}. 

Previous work has also used a \emph{workflow} approach to the network structure inference problem which maximizes performance of particular task(s) on the inferred network \cite{DeChoudhury:2010:IRS:1772690.1772722, Farine2016}. Consider interaction networks over varying thresholds $\tau$. A naive solution for this type of approach is to explore the parameter space of $\mathcal{R}(\mathbf{D}, \tau)$ and evaluate the task performance on each inferred network. However, this is very costly, especially as $\mathcal{R}$ requires more parameters. 

The joint optimization for network structure inference learns the features in $\mathbf{D}$ that perform well at task $\mathcal{T}()$. For example, previous work has learned network models which jointly discovers features in a supervised LDA model, and the logistic regression weights which perform well for an edge prediction task \cite{McAuley:2015:INS:2783258.2783381}. In Equation \ref{eq:joint_opt}, we have already formulated joint optimization network structure inference within our framework, repeated here:
\begin{equation} 
	\label{eq:joint_opt2} 
	\argmin_{\mathbf{G}} e(\mathcal{T}(\mathcal{R}(\mathbf{D}, \mathbf{\alpha}), \mathbf{\beta}), \mathbf{E}^*)
\end{equation}

The jointly optimized model may avoid discovering spurious relational model parameters which are not suitable for the intended task. Second, we may be able to learn a more interpretable relationship between the original feature space and the task model. However, this strategy has the added requirement that the output of each model can be used to re-train the other. For example, \citet{McAuley:2015:INS:2783258.2783381} use a \emph{supervised} LDA model which uses the output of the edge prediction task to re-train the relational model. Because of this added modeling complexity, joint models are relatively rare compared with multi-step workflows.



\subsection{Hypotheses and Tasks on Inferred Networks}

Before discussing data models, we should first have some intuition of what a researcher wants to \emph{do} with the network. Figure \ref{fig:datascience} (right) illustrates the core novelty in machine learning and data science in hypothesis generation, model development, and testing. In machine learning, there is typically a bias toward evaluating these hypotheses using a novel prediction task model. However, typically these models do little to explain the underlying system, and are more useful for generating new hypotheses. In the statistics domain, there is a bias toward descriptive modeling, where the `task' is parameter inference on an assumed parametric (or ``non-parametric,'' \cite{Wasserman:2006:NS:1202956}) statistical model on the data. These parameters are useful at interpreting the underlying system, such as fitting the exponent of degree distributions, or reporting other aggregate statistics on a network. 

Applications driven by descriptive models aim to reconstruct and describe the underlying relational structure with the greatest fidelity, relative to the domain knowledge base. A typical example in this area are gene regulation networks (GRNs). These networks are inferred on data measuring individual genetic expression over different experimental settings. In these networks, nodes represent genes or functional gene families, and edges represent inferred positive or negative gene expression relationships (e.g. ``gene `A' reduces the expression of gene `B' under some context''). Inference of these networks typically identifies new, high quality \emph{candidate} regulation relationships given high accuracy of inferring known edges. These interactions can be experimentally tested to build greater understanding of cellular processes and to develop potential personalized medical treatments.  

In contrast, predictive methods aim to discover topology within the network which maximizes predictive performance, and may not reconstruct the underlying process with the highest fidelity, but with a focus on those aspects or modalities which are most predictive.  Modeling the predictive aspects of the data allows researchers to learn regular relationships between modalities (e.g. call, SMS, and location in mobile phone data) or over time (e.g. periodicities) and aids further hypothesis generation to explain the predictive relationships. However, often highly predictive relationships are also uninteresting and can drive the structure of the inferred network. Domains such as climate tend to remove known periodic dynamics as preprocessing on the underlying data, prior to inferring the network structure.


% \subsection{Problem Definition}
% \label{sec:def}

% We introduce a brief, high-level formalization of the network inference problem. This is intended to provide some precision of elements related to network inference, not necessarily a novel or sufficient expression of the problem.  

% \subsubsection{Preliminaries}

% We define a network $G = \langle \mathbf{V}, \mathbf{E}, \mathbf{A}\rangle$ as a tuple containing a set  $\mathbf{V}$ of $n$ nodes, $|\mathbf{V}| = n$, a set $\mathbf{E}$ of $m$ node pairs $e_{ij} \in \mathbf{E}, |\mathbf{E}| = m$, and set $\mathbf{A}$ containing node or edge attribute sets. A particular attribute, the weight of an edge $w_{ij}$ is a scalar value, $|w_{ij}| \leq 1$, where $w_{ij} = 0$ denotes the absence of an edge. An unweighted network is a special case of a weighted network where $w_{ij} \in \{0, 1\}$. Edge and node \emph{features} are a particular type of attribute, derived by a kernel function measuring some local edge or node property (e.g. node degree). Time-varying network definitions are simply a $t$-length sequence of static network snapshots: $\mathbf{G} = (\mathbf{G}_1,...\mathbf{G}_k,...\mathbf{G}_t)$. 

% \begin{table*}[t]
% 	\small	
% \begin{tabular}{|p{.10\textwidth}|p{.85\textwidth}|}\hline

% \emph{Symbol} &	\emph{Definition} \\
% \hline
% $\mathbf{D}$ & A dataset for input to a network inference method,(temporal, spatial, multi-variate etc.)   \\ \hline
% $\mathbf{G},\mathbf{E},\mathbf{V},\mathbf{A} $ & $\mathbf{G} = \langle\mathbf{V},\mathbf{E},\mathbf{A}\rangle$, an attributed network with nodes $\mathbf{V}$, edges $\mathbf{E}$, and attribute-set $\mathbf{A}$ \\ \hline
% $n,m$ & $n$ number of nodes and $m$ number of edges on network $G$. \\ \hline
% $v_i, e_{ij}, w_{ij}$ & node $v_i \in \mathcal{V}$, edge $e_{ij} \in \mathbf{E}$, edge weight $w_{ij}$ \\ \hline
% $\mathcal{R}() , \mathcal{T}()$ & A network data model function $\mathcal{R}(\mathbf{D}, \bullet) \rightarrow \mathbf{G}$ producing graph $\mathbf{G}$ from input data $\mathbf{D}$, a task model $\mathcal{T}(\mathbf{G},  \bullet) \rightarrow (p_1, p_2...)$ producing a stream of responses from input graph $\mathbf{G}$.\\ \hline
% $e()$ & An error function $e()$ evaluating a task $\mathcal{T}$().\\ \hline 
% $\tau$ & Edge similarity threshold for inclusion in the inferred network, $\tau \leq w_{ij} \Leftrightarrow e_{ij} \in E$ \\ \hline
% %$\tau_{i}$ & The infection time of node $n_i$ (see Section \ref{sec:cascades}). \\ \hline
% %$\Delta_{j,i}$ & The time difference between infection times: $\Delta_{j,i} = \tau_i - \tau_j$. \\ \hline
% %$c, C$ & A cascade, or sequence of infection times of variable length $k: c = \langle \tau_{\alpha_1}, \tau_{\alpha_2}, ..., \tau_{\alpha_l} \rangle$ for some arbitrary index sequence $\alpha; \alpha \in 1...N$. $c \in C$, a set of cascades.\\ \hline
% % $\gamma$ & The algorithm input parameter for initial minimum distance threshold. \\ \hline
% % $k$ & The algorithm input parameter determining the number of top-\emph{k} nearest neighbors to find. \\ \hline
% % $n_k$ & $n_k = nn_k(q, D)$, the \emph{k}-th nearest-neighbor, i.e. $dist(q, n_1) \leq...\leq dist(q, n_k) \leq dist(q, D \backslash \{n_1, n_2...n_k\})$.\\ \hline
% % $e_{i,j} $ & $e_{i,j} = E(dist_{lev}(d_i, d_j))$, the \emph{operations} executed in the $dist_{lev}(d_i, d_j)$ dynamic programming matrix filling. \\ \hline
% % $pp$ & Aggregate pruning power across the entire matching procedure: $pp = 1 - \frac{\sum{e_{i,j}}}{\sum{e_{i,j}^*}}$. \\ \hline
% \end{tabular}
% \centering
% \caption[Definitions]{Table of symbol definitions used throughout this survey.}
% \label{tab:definitions}
% \end{table*}




% The Network Topology Inference problem represents some input data as a network and \emph{validates} this network relative to performance on some task(s). This is an active area of research across many application domains, but lacks a general framework for evaluation, typically using domain rules-of-thumb and application-specific evaluation schemes. This is an initial work formalizing this problem, particularly in the absence of ground-truth network data.

% The network topology inference problem combines two basic models: first, a \emph{network model} $\mathcal{R}(\mathbf{D}, \bullet) \rightarrow \mathbf{G}$ constructs network $\mathbf{G}$ on input data $\mathbf{D}$. This model may be parametric statistical models (e.g. ERGMs) or non-parametric and threshold-based interaction networks. Second, the problem uses a \emph{task model} $\mathcal{T}(\mathbf{G},  \bullet) \rightarrow (p_1, p_2...)$ on input $\mathbf{G}$ under some parameters, which emits task responses (e.g. prediction `$p_i$'). These responses approximate the hidden, ideal function $\mathcal{T}^*(G)$ of a particular network task (e.g. classification, prediction) with error $e()$. 



\subsubsection{Summary}

In Table \ref{fig:citations} (Column `Model'), we label these models under two broad categories. First, \emph{parametric models} allow interpretable, descriptive statistics.  We identify graphical models (\textbf{GM}) and other network models fit with maximum likelihood methods (\textbf{ML}), relative to some assumption on the input data such as information flow between nodes \cite{Gomez-Rodriguez:2012:IND:2086737.2086741}. Causal models (\textbf{CM}) typically generate causal networks--a special case of graphical models--using Granger causality \cite{Granger1969} or other causal definitions \cite{Meek:1995:CIC:2074158.2074204, PMID:15360909}. These networks represent strong relationships between nodes which control for confounding factors caused by other (possible) adjacent nodes. 

Second, \emph{non-parametric models} tend to directly measure interactions between nodes and use statistical tests to determine appropriate edge weights. Section \ref{subsubsec:interaction} covers this category in greater detail. We categorize work related to novel and `ad-hoc' interaction measures (\textbf{I}) between the data associated with pairs of nodes, correlation networks (\textbf{IC}) which measure linear, cross, or some other correlation, entropy (\textbf{IE}), frequency domain measures (\textbf{IF}), and regression (\textbf{R}).



% \subsection{Methods for Network Structure Inference}

% We organize related work broadly along the type of network structure inference \emph{model} used, including parametric, non-parametric and various thresholded interaction/correlation measures. Within these groupings, we categorize the type of task performed on the network, including edge and attribute prediction, descriptive analysis, or model selection. 

%Table \ref{fig:citations} summarizes work across several domains, introducing the basic scientific question driving the analysis, and the network structure inference model used to realize the network. 



  


%============================================
%=================EDIT=======================



\subsection{Evaluating Networks and Tasks}

Evaluation strategies over the entire workflow of Figure \ref{fig:datascience} measure the performance of the \emph{final task} (prediction or statistical inference). In this context, the network serves as a model of the data, but the fidelity of this model in terms of fitting error, or evaluation against partial ground truth network data does not measure the network's usefulness at answering questions on the original input data. For any non-trivial data or domain, it is perhaps more appropriate to think of the space of networks as \emph{possible} representations with some utility for answering a specific question. `The network' is typically seen as uncovering the true relational structure of the data with some error \cite{Wang2012396}. 

Most scientific domains agree with an evaluation strategy focused on final task (a network \emph{for} location prediction, brain activity response etc.), because there is no validation data for evaluating the inferred network structure directly. For example, we simply cannot survey baboons \cite{Farine2016} as we can humans \cite{Eagle2009} to discover their real friendships. Furthermore, uncovering the general, robust network from complex data may not appropriately model the overlapping modalities of the data. For example, a multitude of contexts might mean that functional brain networks are inherently probabilistic and extremely context-dependent. Discovering a general representation across these contexts will be less informative because it does not account for this complexity. 


This formulation may seem underspecified. However, it succinctly clarifies the relationships between data input, the network model, and the task model. It explicitly formulates network $\mathbf{G}$ as a \emph{model} on data $\mathbf{D}$ for task $\mathcal{T}^*$, approximated by $\mathcal{T}$. This formulation captures simple \emph{interaction network} workflows (see: Section \ref{subsubsec:interaction}) which separately infer the network (often by expertly-tuned thresholds) and validate task performance, as well as parametric inference methods which learn the network model parameters (and possibly, jointly the task model parameters). To our knowledge, all network inference models can be formulated in this pattern, and all network inference models \emph{should} be formulated relative to a particular task or hypothesis. In much of the existing work, the network model or task model will not be formulated explicitly, or the space of possible model combinations may be under-explored.

We can instantiate several tasks within this framework. In the context of network prediction tasks, our predictive model can output predictions of (1) edges, (2) attributes, or (3) the original data. For one instantiation, on a validation edge-set $\mathbf{E}^*$, we can evaluate:
\begin{equation} 
	\label{eq:joint_opt} 
	\argmin_{\mathbf{G}} e(\mathcal{T}(\mathcal{R}(\mathbf{D}, \mathbf{\alpha}), \mathbf{\beta}), \mathbf{E}^*)
\end{equation}	

This is a joint optimization of $\mathbf{G}$ over parameters $\alpha$ and $\beta$, for edge prediction. In this context, the suitability of both the network and task models (and the appropriate error function) will determine the performance of the inferred network. This joint model may an EM-like formulation, where the task and network models share information iteratively to re-learn their parameters. 

This formulation also demonstrates two key challenges in the network inference problem. First, the parameter space of possible $\mathbf{G}$ from $\mathcal{R}(\mathbf{D}, \bullet)$ may be large, and the joint optimization with the parameters of a given task is likely to be non-convex. Furthermore, well-performing local solutions in the task parameter-space may have different network topologies. Summarizing and reconciling these differences may be important in interpreting where the network is most robust. It is unclear how to reconcile differences  and summarize this space of \emph{plausible} networks into a single, interpretable, effective model. This proliferation of possible task and network model combinations makes further hypothesis generation and testing daunting for the researcher, who has diminishing confidence in empirical statements about the system of interest.

\subsubsection{Summary}

Table \ref{fig:citations} (Column `Task') categorizes rows within each domain by the type of task performed, under the caveat that one study may use several evaluation strategies, or that the actual task could only loosely be described as the canonical task (e.g. edge prediction). 

First, we denote predictive tasks, including edge prediction (\textbf{PE}) and attribute prediction (\textbf{PA}). Attribute prediction can also describe prediction of the original data. Predictive models are relatively rare across domains because researchers are very interested in expressive models which give insight into the underlying system. We observe some specialization in both information networks (in the machine learning literature) and epidemiology, which aims to predict the extent or timing of an epidemic over a population in varying contact models. 

Second, descriptive analysis is broken into node-oriented statistics (\textbf{DN}), this includes reporting distributions of simple node statistics including degree distribution, clustering coefficient, correlation distributions, etc. This often constitutes the base-level exploratory analysis. Role-oriented analysis (\textbf{DR}) aims to characterize nodes using network features, by the structural roles they play in the system (\emph{i.e.,} bridges in-between social communities). Other high-order analysis (\textbf{DH}) examines communities or other larger subgraph structures beyond node and edge-based descriptive statistics. 

In both descriptive and predictive cases, we observe a good deal of work in model selection (\textbf{MS}). These varying models correspond to different hypotheses to how the network might have been generated.

%============================================
%=================EDIT=======================





%  In Figure \ref{fig:taxonomy} (2A) we define the pattern of these models as \emph{coupled} inference-prediction models. In the absence of both evaluation network data and an assumed underlying network model to fit, existing methods have relied on a prediction paradigm to infer network networks with low error for some prediction task (Figure \ref{fig:taxonomy} (2B) is empty because descriptive methods require some model assumption or reference network). These methods validate the inferred network network $\mathbf{G}$ on hold-out input data $\mathbf{D}'$, auxiliary node-attribute set $\mathbf{A}$, or the network topology itself (e.g. at a different time, for dynamic networks). 

%Most domains of science using network inference have a lack of `ground truth' data due to the nature of the applications studied. For example, we cannot know the `true' social network of an animal population. Rather, social animals likely do not have one true social network describing behavior or decision-making, but several networks on differing tasks, activated by context. The coupled paradigm directly models these motivations, which generalize to many domains lacking true ground truth networks. Simple thresholding and similar paradigms which infer `the' single network are prone to confuse overlapping relational contexts within the input dataset.   





%

% an expert-tuned threshold of some pairwise similarity measure between nodes (e.g. correlation, mutual information).  Recent work reiterates the assumption that: ``inferring networks from pairwise interactions cell-phone call or email records simply reduces down to selecting the right threshold $\tau$ such that an edge (u, v) is included in the network if u and v interacted more than $\tau$ times in the dataset. Similarly, inferring networks of interactions between proteins in a cell usually reduces to determining the right threshold'' \cite{Myers2010}. However, these subjective thresholding choices may produce very different subsequent analysis and may lead to incorrect or incomplete conclusions. All of the below paradigms may in fact use simple thresholding as the mechanism for constructing the inferred network, possibly globally tuning the edge definition threshold relative to sampling some subsequent error performance.


%\subsection{Design Patterns}

%The latent network construction problem has been especially relevant in scientific discovery in such domains as bioinformatics \cite{Dhaeseleer2000}, neuroscience \cite{VanWijk2010}, climate informatics \cite{Tsonis2004497}, ecology \cite{Milns2010} and many others. We select a subset of these domains to give a

%In this section, we dig deeper into each cell in the Figure \ref{fig:taxonomy} taxonomy to describe several common patterns across domains.  

%provides example design patterns of each cell of the matrix according to their differing types of tasks and evaluation data.



%\subsubsection{Correspondence}



%\subsubsection{Stand-alone}



%\subsubsection{Model fitting} 



%\subsubsection{Coupled inference-prediction}




%%% to incorporate
%Previous work demonstrated this paradigm as a proof-of-concept \cite{DeChoudhury:2010:IRS:1772690.1772722}, \emph{coupling} latent network inference and prediction using simple node features. Our work extends this proof of concept, describing a framework to measure and tune network inference parameters according to behavioral prediction on nodes \cite{Farine2016}. This work explores simple thresholding network inference methods on a dataset $\mathbf{D}$ of geo-social data sensing social interactions of a troop of baboons. Loss $\mathcal{L}(\mathbf{G} | \mathbf{D'})$ is evaluated on hold-out data by imputing individual locations using queried network topology of $\mathbf{G}$. This work demonstrates that predictiveness using simple thresholding may gradually degrade relative to the threshold. This yields a trade-off between edge quality and coverage, depending on the tolerance for errors in the subsequent task.

%Our work focuses on the case (2B), where we infer predictive networks largely in the absence of a known ground-truth. The accuracy of these networks is measured in the capability to predict node behavior over time.   

%Similar work has provided empirical results for injected noise in known networks \cite{Wang2012396}. 


%Typically, the network model is not fit against the evaluation network data, $\mathbf{G}'$ in the inference phase.   We do not typically find that these  observe  We generally observe that model fitting methods do not incorporate 

%Section \ref{subsec:coupled} describes an emerging paradigm in network analysis using a  which tunes the network definition over a parameter space in order to optimize for the (generalizable) performance of a subsequent task. This area of analysis may furthermore yield multiple, ``alternative'' views of the prediction task, analogous to the concept of ``alternativeness'' in clustering \cite{Qi:2009:PFF:1557019.1557099}.  




%Figure Section \ref{sec:cascades} gives a detailed overview of current work in the \textbf{cascade} workflow. This work focuses on network construction where we can observe only information arrival at nodes, but the edges used in transmission are hidden. 


%The key distinction with other applications is this design pattern predicts between two different modalities,  the stand-alone workflow is that these analyses aim to ultimately demonstrate that the correspondence is predictive across modalities. These methods differ from the simple thresholding workflow because the ground truth network of the other modality may be used to tune or verify the latent network model. % predictive activity the use of cell phones exists when there is an evaluation dataset such as an explicit 

%In the presence of  ground truth,









%Especially within the predictive paradigm, we will dig deeper into the statistical tests used, which are diverse depending on the applications. These methods typically use (i) pairwise similarity measures, regression, or similar pairwise comparisons to define edges, (ii) optimization functions which have fit to an expected higher-order structure (e.g. information diffusion) or . 

%In the latter case (), researchers make some topological assumptions about the inferred network and show that the underlying data fits these assumptions. Several papers exist which infer the maximum likelihood network from a dataset of ``hitting time'', where each node is ``infected'' at some timestamp \cite{ICML2011Gomez_354}. This work is evaluated against a known network to emit hitting times, and uses network reconstruction by learning the underlying transmission likelihood; these methods largely fall within the descriptive maximum-likelihood methods with evaluation data (1A). 

%We further examine these evaluation methods in the absence of evaluation network data. existing network inference work by the type of evaluation in the absence of evaluation network data.

%: (1) aids researchers in interpreting ``why'' entities have an edge relationship in terms closer to the domain knowledge-base, for example, directly from loss-optimization, $\mathcal{L}(\mathbf{G} | \mathbf{D})$. (2) may not fully represent the relational structure, simplify it for maximizing predictive performance, e.g. tuning $\mathbf{G}$ using $\mathcal{L}(\mathbf{G} | \mathbf{D'})$ according to hold-out data $\mathbf{D'}$. An edge in this network exists because it predicts $\mathbf{D'}$, leading to further hypothesis generation and testing for this relationship. 

%This split emphasizes that (1) does not make assumptions about higher-order structure and may produce spurious network measures depending on edge quality, and (2) tend to optimize for a specific network feature and may give poor results when these modeling assumptions are violated. No known network construction method quantifies uncertainty across simultaneous network measures.  

%Second, we categorize methods based on validation procedures using: 

% \begin{enumerate}
% 	\item  
% 	\item  
% \end{enumerate}

%%%%$% This looks at existing work in latent network construction on two important axes. First, we split previous work according to \textbf{predictive} and \textbf{explanatory} models. An explanatory model aims to accurately describe the relational structure of the underlying data, and give some insights to the rules which 

% We look at  In rare cases such as gene regulatory networks, the end-goal is the 
% 
% This is an informative split because (1) does not make any assumptions about higher-order structure and may produce spurious network measures based on uncertainty, depending on thresholding , while (2) generally does 




%    one particularly important pattern is  In Section \ref{subsec:known} we examine work focused on reproducing the relational, experimental domain knowledge in contexts such as gene regulatory networks (GRNs). 
% 
% 
% In this problem setting, With some simplification, this can be called the \textbf{stand-alone} workflow for latent network construction, where the final purpose of the inference is largely the network itself. 
% 
% 
% This is a popular modeling choice because it allows researchers to borrow from a mature set of relational analytical tools for networks. We will look at several patterns related to how these networks are used. 
% 
% Section \ref{subsec:thresholding} looks at a typical case where no ground truth network is available.






%old fig:
% \caption{An overview of the patterns of workflows for latent network construction within the survey taxonomy}
% \label{fig:taxonomy}
% \end{figure}
% 
% \begin{figure}
% 	\centering
% \begin{tabularx}{.90\textwidth}{ r|X|X| }
% \multicolumn{1}{r}{}
%  &  \multicolumn{1}{c}{(A) Predictive}
%  & \multicolumn{1}{c}{(B) Descriptive} \\
% \cline{2-3}
% (1) Evaluation Network & Correspondence \newline $\mathcal{F}(\mathbf{D}):= arg\,min_\mathbf{G}\  e(\mathcal{P}(\mathbf{G}, \mathbf{G}^*))$ & Stand-Alone \newline $\mathcal{F}(\mathbf{D}):= arg\,min_\mathbf{G}\  e(d(\mathbf{G}, \mathbf{G}'))$ \newline Model fit (e.g. cascades) \newline $\mathcal{F}(\mathbf{D}):= arg\,min_\mathbf{G}\  e(fit(\mathbf{G}, \bullet))$  \\
% \cline{2-3}
% (2) No Evaluation Network & Coupled (data) \newline  $\mathcal{F}(\mathbf{D}):= arg\,min_\mathbf{G}\  e(\mathcal{P}(\mathbf{G}, \mathbf{D}'))$ \newline Coupled (self) \newline $\mathcal{F}(\mathbf{D}):= arg\,min_\mathbf{G}\  e(\mathcal{P}(\mathbf{G}_t, \mathbf{G}_{t+k}))$ & -- \\
% \cline{2-3}
%   & \multicolumn{2}{|c|}{Simple thresholding}\\
% \cline{2-3}
% 
% \end{tabularx}
% 
% \caption{An overview of the patterns of workflows for latent network construction within the survey taxonomy}
% \label{fig:taxonomy}
% \end{figure}



% \begin{figure}
% 	\centering
% \begin{tabularx}{.90\textwidth}{ r|X|X| }
% \multicolumn{1}{r}{}
%  &  \multicolumn{1}{c}{(A) Predictive}
%  & \multicolumn{1}{c}{(B) Descriptive} \\
% \cline{2-3}
% (1) Evaluation Network & Mobility & Gene Regulatory Networks, Epidemiology \\
% \cline{2-3}
% (2) No Evaluation Network & Climate, Ecology & -- \\
% \cline{2-3}
% \end{tabularx}
% \caption{A summary of contexts for network structure inference across applications}
% \label{fig:taxonomy_top}
% \end{figure}
% %\caption{test}
% %\vspace{15px}
% 
% \begin{figure}
% 	\centering
% \begin{tabularx}{.90\textwidth}{ r|c| }
% 	  \cline{2-2}
% 	   \multirow{2}{*}{Relational data models}  & i. Association Networks \\
% 	 	\cline{2-2}
% 	   & ii. Maximum-Likelihood Networks \\ 
% 		\cline{2-2}
% 	   & iii. Joint-optimization Networks \\
% 	\cline{2-2}
% \end{tabularx}	
% \caption{A summary of relational data models for network structure inference}
% \label{fig:taxonomy_bottom}
% \end{figure}
%
% Along a second axis, network inference methods are validated using:
% 
% \begin{enumerate}[label=(\Alph*)]
% 	\item Ground-truth networks and/or synthetic network models.
% 	\item Statistical tests in the absence of ground-truth networks and an assumed synthetic model. 
% \end{enumerate}


% \begin{enumerate}
% 	\item Descriptive models representing the underlying relational structure with the greatest fidelity.
% 	\item Predictive models using the inferred network as a data representation for prediction, maximizing performance of the subsequent analysis.
% \end{enumerate}


%In (A) the evaluation strategy is straightforward: we directly measure the agreement with the ground truth or synthetic network. These evaluation strategies assume that the process generating node interactions in the input dataset is equivalent to the evaluation network (see Section \ref{subsec:interaction}). The evaluation strategies for (B) are more diverse in the literature. Three predominant tests include (i) randomization tests or null modeling which measure the significance of a given edge, (ii) information-theoretic measures such as entropy, and (iii) joint optimization which balances cost and utility.

%as models on underlying data,  to think of We propose that there is not the `true' network on any non-trivial data or domain, but a range of network representations 



%solves some task(s) by applying through an intermediate, learned network topology.  The Latent Network Inference problem aims to construct and \emph{validate} a latent network network representation.  

% problem formulates a relational data model  to solve task . 


%and an error function $e_\mathcal{T}(\mathbf{G})$ on input data $\mathbf{D}$, . The error function $e()$ formulates the desired properties of the network model $\mathbf{G}$ to satisfy some \emph{task} $\mathcal{T}$. This formulation generalizes inference methods which use maximum likelihood fit or similar optimization $\mathcal{F}(\mathbf{D}):= arg\,min_\mathbf{G}\  e(fit(\mathbf{G}, \bullet))$ for some parametric model, as well as prediction-based models which hold out a $\mathbf{D'}$ for a different time, place, or modality, $\mathcal{F}(\mathbf{D}):= arg\,min_\mathbf{G}\  e(\mathcal{T}(\mathbf{G}, \mathbf{D'}))$, or an evaluation network $\mathcal{F}(\mathbf{D}):= arg\,min_\mathbf{G}\  e(\mathcal{T}(\mathbf{G}, \mathbf{G}'))$. 




%This is an active area of interest across application domains, but largely lacks a framework for evaluation criteria of a “good” network other than by application-specific strategies and rules of thumb. This is an initial work for formalizing the evaluation of this problem, particularly in the absence of ground-truth network data.

%$c = \langle \tau_{\alpha_1}, \tau_{\alpha_2}, \tau_{\alpha_k} \rangle$ of variable length $k$

% \begin{figure}[h]
% \centering{\includegraphics[width=0.75\columnwidth]{figs/model}}
% \caption{The common network construction workflow.}
% \label{fig:model}
% \end{figure}

%N and construct unweighted edges $\langle n_i, n_j \rangle \rightarrow \{0 , 1\}, i \neq j, n_i \in V \land n_j \in V$ between pairs of individuals (i.e. nodes) based on two network inference procedures:

==> conclusions.tex <==
\section{Conclusions and Future Work}

==> intro_old.tex <==
\section{Introduction} \label{sec:intro} 

\footnote{NOTE: I'm happy to use ``Network Construction'' in place of latent network inference. It's clearer to me.} Using networks as a model to understand natural systems transcends most branches of science and engineering. The capability for networks to model the complexity of these systems has given rise to ``network science,'' the development of rigorous understanding of the shared properties of networks across their many applications, \cite{Barabasi2012, ARIS:ARIS1440410119}. 

In many network science applications, the definition of the network is not explicit, but inferred from non-relational data, where the edge definition represents a latent relation between two nodes. Though much work has been dedicated to network models and their properties, the correctness of latent network definitions is not well understood. Therefore, \emph{how} to best infer a network while incorporating constraints and assumptions of the application is an open problem in network science.

\subsection{Problem Definition} \label{subsec:problem_def} A latent network contains nodes or edges which have been inferred from a set of features. Inferred nodes represent actors or functional units, while inferred edges represent some relationship between nodes. One or both of nodes and edges may require an inference step. A network inference function takes as input the data feature-set, and outputs an $N x N$ weighted or binary adjacency matrix (for $N$ inferred or fixed nodes). 

The term `network inference' is used in several contexts. Our use of `network inference' is related to the network construction: the edge and node definitions from non-relational data. Other uses of `network inference' may refer to discovering missing edges or nodes (under a fixed network definition), or any other missing-value `inference' for node/edge attributes on a given network structure. 

\subsection{Challenges} \label{subsec:challenges}

\footnote{NOTE: I have some text for this but needs work. I'll try the bulleted version} Measuring the \emph{quality} of an inferred network is a difficult problem because: 
\begin{itemize}
	
	\item A node or edge in a latent network often represents a complex statistical relationship, yielding a large space of plausible networks 
	\item Researchers rarely have ground truth to validate the inferred network 
\end{itemize}

%The meaning of a node or edge in a latent network is often a complex statistical relationship. Consequently, measuring the \emph{quality} of an inferred network is a difficult problem. One simple evaluation found in the literature [citation needed] is to compare against expected network statistics (e.g. degree distribution, average clustering coefficient), tuning the network inference parameter(s) to these assumptions. However, these global statistics describe a large space of possible networks [citation needed], and the correctness at a micro-scale (e.g any given edge) is not assured. Another evaluation [citation needed] looks at parameter sensitivity of the network inference method. However, if the parameters have any effect, they will generate a space of plausible networks
NOTE: sensitivity analysis figures go here to motivate instability of results to the construction step.

\subsection{Our Contributions} \label{subsec:contributions}

We organize network science research across nine different domains: bioinformatics, climate and environmental science, communication networks, ecology, economics, epidemiology, mobility and mobile computing, and neuroscience. In each of these domains, researchers often infer networks from non-relational data sources. We organize this work from a computational perspective, tracking the similarities of methods and datasets across domains and contrasting the assumptions which guide the network inference procedure. 

Our survey is the first to organize such a large, multi-disciplinary body of research from the computational perspective with a particular focus on the \emph{network definition} procedure. There exist many reviews in statistical network modeling which focus on models and measures of networks (e.g. \cite{Goldenberg:2010:SSN:1734794.1734795, Lü20111150}) and broad network science surveys (e.g. \cite{Havlin2012}). However, these do not focus specifically on network construction. Several recent domain-focused meta-studies \cite{Marbach2012} or surveys in bioinformatics \cite{PMID:17981545, Yu2013, Hecker200986, Barabasi2004}, ecology \cite{Krause2013}, neuroscience \cite{Bullmore2009, simpson2013} all have some discussion of network construction specific to the domain. However, none of these have network inference as a specific focus, and are limited to discussion of the single domain. 

To our knowledge, the most similar work to this survey is \cite{Kolaczyk2009}. The author organizes work in three different categories: (1) link prediction, where some edges and all nodes are known and the task is to infer new edges, (2) association networks, where all nodes are known, and the task is to infer edges (e.g. by correlation), and (3) network tomography, where some edges and nodes are known, and the task is to infer `interior' (unobserved) node and edge topology. Of these, only (2) is similar to our work; we focus with greater depth on the network construction procedure, where no edge definition is known a-priori. Furthermore, we organize a broader, multi-domain collection of research by data characteristics and methods, facilitating cross-domain investigation.

\subsection{Organization} \label{subsec:organization}

\footnote{NOTE: I generally don't like these at all, and never read them, but for the sake of an outline and to test my label anchors...} This survey is organized as follows: Section \ref{sec:problem} describes the latent network inference problem in detail, including the Section \ref{subsec:framework} introducing the general latent network framework, and Section \ref{subsec:organization} organizes and visualizes the current work across the surveyed application domains. Section \ref{sec:applications} presents problem formulations in each domain application, and several of data aspects and domain assumptions which motivate the methods arising for each application. Section \ref{sec:conclusion} concludes by summarizing key considerations for network construction. 


==> junk_pile.tex <==

%%%%%%%
%FROM: introduction_wcp.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%When this underlying dataset has no unambiguous network structure defined on it In many cases, this construction step is difficult because the edge definitions must be learned, and these statistical relationships


%going from an underlying dataset Representing the collection of ``Friend'' relations between users as a network is a trivial task The \emph{construction} of these networks is trivial because the underlying ``friendship'' 



%%%%%%%
%FROM: work.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%information passing through a hidden network and the task  




% The network construction step is typically the incorporation of domain assumptions and parameters, . However, little work has explored how the space of plausible networks can be used to understand   for analysis. Rather than However rarely  , while we will see in many cases 
% 
% 
% We will look at current research 
% 
% 
% 
% Domains vary greatly inthe application and sophistication of network construction methods. For example gene regulatory network (GRN) inference is a very mature area because of the availability of a verified ground truth network of gene regulation. The inference task then becomes reproducing 
% 
% 
%  Much of the domain practitioner's work from data to a network model is incorporating the domain knowledge which will yield an a-priori threshold  to get from raw data to a network is  Much of the application of ``data science'' is scattered across these domains, and often this network construction step will be the incorporation of domain knowledge for edge definition and construction,  work in the construction of networks is scattered



% \subsection{Parametric network fit 1}
% 
% \cite{Angluin2013}
% 
% \subsection{Parametric network fit} \todo{2A, find this}
% 
% \cite{friedman2010applications,liu2011learning}


%------------------------ 
%FROM: work_cascades.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%\cite{ICML2011Gomez_354}, \cite{Gomez-Rodriguez:2012:IND:2086737.2086741}, \cite{Cho2011,Myers2010}

  %defined by: $k(\tau_l, tau_i) = exp()$ Having kernelized the hazard function, we then 

%Figure \ref{fig:diffusion} \todo{return}

%This work is further extended in \cite{NIPS2012_4582} where the authors learn non-parametric \todo{fill this}.

%introduces a probability model 


%$P_c(n_i, n_j)$ for incubation between nodes. The authors define exponential and power law models on the difference in infection times, $\Delta{i,j} = \tau_{j} - \tau_{i}$:



% \begin{equation} \label{eq:leskovecexp}
% P_c(n_i, n_j) = P_c(\Delta_{i, j}) \propto e^{-\frac{\Delta_{i, j}}{\alpha}} 
% \end{equation}
% 
% \begin{equation} \label{eq:leskovecpower}
% P_c(n_i, n_j) = P_c(\Delta_{i, j}) \propto \frac{1}{(\Delta_{i, j})^\alpha}
% \end{equation}



%The authors use an independent Bernoulli process rather than an infection model which varies by time, this may not correctly model propagation in applications where susceptibility changes by time. 
%Generating a dataset These \emph{cascades} (or paths)  of variable length $k$  Using this incubation model, we can generate Querying this model, we  relative to an incubation model infection ach node  propagation times.  the specific attempts to Given a list of propagation One well-established line of work infers a network based on the most likely




%This is essentially equivalent to the ``support'' of spanning trees  The algorithm is able to produce these neighborhood sets only on the first edge (e.g. first edge) of a trace

% \begin{equation} \label{eq:abrahao_score}
% S_{max}(n_i) = \argmax_{S}\sum\limits_{c \in C}\left( log |S_c| - \lambda \sum\limits_{j \in S_c}\Delta_{j,i} \right)
% \end{equation}

% Equation \ref{eq:abrahao_score} finds a subset $S$ maximizing the log size of $S_c$ against the total transmission likelihood over each interval $\Delta_{j,i}$ for a fixed transmission rate $\lambda$, where $S_c = \{v \in S | \tau_v^c < \tau_i^c\}$. Note that $\tau_v^c= \infty$ when $\tau_v \notin c$, therefore the construction of each $S_c$ 

%building an arbitrary subset $S$ relative to $n_i$ which , scoring the sum of $log(|S_i|) - \Delta_{j,i}$ on $S_i$, across all cascades.  These likely `neighborhoods' of each $n_i$ are used to output edges. 

 %which builds a subset candidates which an arbitrary set %$S_c = \{v \in S | \tau_v^c < \tau_i^c\}$ which maximizes: 
%   on $n_i$ which essentially selects minimum spanning trees   , for each cascade $c_l, l = 1...|C|$   , scoring arbitrary, enumerated subsets on cascade $l$,  based on their relative infection times to $n_i$: 


% 
% Equation \label{eq:abrahao_score} essentially selects a subset $S$ relative to $n_i$ which maximizes the difference of the log size of the subset vs. the sum of $\D_{j,i}$ over all $j$. Note that S_c is constructed


%raise concerns about the higher-level structure of the networks have raised large questions about the higher-level structure inferred using these methods. \ref{Abrahao:2013:TCN:2487575.2487664} give several approximation guarantees relative to the number of cascades, $|C|$. The authors 

%\ref{Abrahao:2013:TCN:2487575.2487664}, \cite{Netrapalli:2012:LGE:2318857.2254783}, \cite{2013arXiv1301.6916G}











%%%%%%%%%%%
%% FROM: work_thresholding.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%these thresholds are plotted  the log density of edges (lighter is more dense). 


% procedure to fix a threshold on the pairwise $P_{ij}$ and $M_{ij}$
%``The edge inclusion threshold for the final network (Section 2.4) was varied in [0;1], and the respective final network for each given threshold was compared with the original net, yieldingSNand SPvalues for the generation of receiver operator characteristic (ROC) curves and area under curve (AUC) values'' \cite{Bender15092010}
%The simple thresholding network construction workflow calculates a set of pairwise similarity a  typically uses some statically-tested or domain informed 
%\cite{Kawale:2012:TSS:2339530.2339634}, \cite{Donges2009}



%%%%%%%%%%
%% FROM: work_prediction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%intro  or  which has neither a strong correspondence to auxiliary ground truth, nor can be informed by  
%The problem of coupled prediction is unique from the other latent network construction workflows examined The examined network construction workflows

%Previous work has focused on defining a network which either (1) was a good representation



%This method measures pairwise weights $w_{i,j}$ between users as the geometric mean of outgoing and incoming communication between $n_i$ and $n_j$. An unweighted, undirected edge-set is constructed using the threshold $\tau$, $\langle n_i, n_j \rangle \in E \Leftrightarrow w_{i,j} \geq \tau$. By increasing $\tau$ the method selects edges with a larger volume of communication over the time period. The collection of networks produced by varying $\tau$ are represented as $\{G_{\tau_1},...,G_{\tau_{K}}\}$. The task is then to


%%%%%%%%%%
% Work interactions.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Crandell text below
% \cite{Crandall2010} also presents an empirical analysis showing that co-located photo events in space and time correspond to `friendship' in the Flickr social network. The authors discretize the geographic space into a fixed grid of cells. The authors define a simple Bayesian likelihood function for friendship given co-location P(``n_i and n_j are friends''| ``n_i and n_j are observed in the same cells $L$ for the last k time-steps''). Although the authors do not explicitly formulate this as a link prediction problem, a maximum likelihood approach seems straightforward for learning an adjacency matrix from the data (see: Section \ref{sec:cascades}). 

% No I'm not using Crandell I hate this paper.
%  \cite{Crandall2010} also presents an empirical analysis showing that co-located photo events in space and time correspond to `friendship' in the Flickr social network. The authors discretize the geographic space into a fixed grid of $S$ cells. We can then define a simple Bayesian likelihood function for friendship given co-location P(``n_i and n_j are friends''| ``n_i and n_j are observed in the same cells $L$ for the last k time-steps''), using Bayes' theorem:
% 
% \begin{equation} \label{eq:colocation}
% P(F|L_k) = \frac{P(F)P(L_k|F)}{P(L_k)}
% \end{equation}
% 
% The prior of two individuals being friends is simply, $P(F) = 1/M$, where $M$ is the number of edges in the explicit network. Although the authors do not explicitly formulate this as a link prediction problem, and use explicit network information in the priors for Equation \ref{eq:colocation}, these might also be estimated from the data. The conditional probability is modeled under the assumption that two friends choose to visit a particular site with probability $\beta$:
% 
% \begin{equation} \label{eq:colocation}
% P(``n_i, n_j are friends and co-located for k time steps'') = p_1^k = (\beta + \frac{1 - \beta}{|S|})^2
% \end{equation}   
% 
% Equation \ref{eq:colocation} has a term $\beta$ for friends jointly choosing the same site, and $\frac{1 - \beta}{|S|}$ for friends `accidentally' choosing the same site at random, where $p_2^k = (1/|S|)^k$ is the likelihood of non-friends choosing the same cell for $k$ time steps, under a naive uniform random selection. The authors introduce a density function for cell selection to improve this, with exponential decay $\gamma$, and introduce a fifth parameter $\alpha$, the likelihood of visiting any cell at this time step, or do nothing. The full likelihood function is parameterized on ($M=7,500, |S|=64,800, \alpha=0.29, \beta=0.12, \gamma=1.8)$. The authors empirically observe $P(F|L_k)$ varying the length of a `time step' (e.g. 1 day, 7 days, 14 days...), and the threshold of co-located events over that time (e.g. analogous to choosing the similarity threshold $\tau$, see Section \ref{subsec:thresholding}).    
% 
% 
% 
% Later work in this area

%% No I'm not using Crandell I hate this paper.
%%%







%in the time-evolving edge set   interval  that exist tests the formation of new edges on the test window $[t+1, T]$: \forall  n_i . The model makes prediction of new edges in the test window [t+1, T]: $\langle n_i, n_j \rangle \notin    over a training window $\omega \leq t$
%The authors construct this network using  by a simple 
%illustrates (A) a weighted latent network constructed from

%In a predictive context, correspondence between two distinct processes allows one to be  Research motivated for discovering correspondence






==> work-cascades.tex <==
\subsection{Network construction from information flow}
\label{sec:cascades}
This line of work uses latent network construction to accurately represent information routing pathways through a set of nodes, when the network topology is unobserved. This area of work borrows terms from epidemiology where we can observe the infection times of individuals, but not the specific contacts which spread the disease. By measuring the likelihood of paths through the sequence of observed infections, the inferred network may be useful in explaining future propagations, or detecting new propagation patterns. This problem formulation is well studied because the spread of information through networks is of tremendous importance across many applications. 

%Early work: \cite{1517844} \todo{fill here}
Figure \ref{fig:diffusion_ex} illustrates the intuition of network construction from propagation through a hidden network $G^*$. Each cascade gives an indication of possible transmission between nodes. The collection of larger cascades builds a more accurate estimation of the network topology. For example, the starting node $n_s$ initiates the spread through the network. However, on our set of three cascades $\{c_1, c_2, c_3\}$ we do not observe the directed edge  $\langle n_s, n_i \rangle$, suggesting that this transmission is unlikely under our cascade set. The key of this network construction task is measuring the quality of cascades, so that many high-quality cascades can recover the underlying transmission network. 

\begin{figure}[h]
\centering{\includegraphics[width=0.50\columnwidth]{figs/new_cascade}}
\caption{Example adapted from \cite{Gomez-Rodriguez:2012:IND:2086737.2086741} demonstrating the intuition of constructing network $G^*$ on a collection of cascades $c_1, c_2... c_k$. For any node $i$ these methods use possible cascades (paths) which include $i$ to estimate the likelihood nodes infecting $n_i$.}
\label{fig:diffusion_ex}
\end{figure}

We will give an overview for the method structure presented in \cite{Myers2010} (named CONNIE) using convex programming, and we look at subsequent analyses using very similar frameworks. The input data for this method is a list of nodes ($n_1, n_2... n_N$), and the infection time of each node ($\tau_1, \tau_2, ...\tau_N$). CONNIE can be used with arbitrary infection models  (\emph{e.g.,} susceptible-infected (SI), susceptible-infected-susceptible (SIS), susceptible-infected-recovered (SIR), see: \cite{bailey1975mathematical}). For simplicity, we describe the susceptible-infected model where a node $n_i$ remains infected indefinitely after receiving the information at time $\tau_i$. The task is to reconstruct the most likely directed tree of information propagation through the nodes. Let the $A$ be a matrix storing the probability of edge adjacency. The authors use an Independent Cascade model where an uninfected $n_i$ is exposed to infection by adjacent node $n_j$ using a Bernoulli process with a fixed probability of infection $A_{j,i}$ at each time step \cite{Kempe:2003:MSI:956750.956769}.  %relative to some incubation model measuring the probability of spread for a difference in infection times: $w(i, j) = P(n_i$ infects $n_j | \tau_j - \tau_i)$. 
Given node infection times, $\tau$, we can generate possible cascades (simple paths) of infection $c = \langle \tau_{\alpha_1}, \tau_{\alpha_2},...,\tau_{\alpha_l} \rangle$ of variable length $l$, where $\alpha$ is a non-repeating subset of indices $\alpha \subseteq \{1...N\}$. This sequence must be monotonically increasing to be valid because each node can only infect another at a later time: $P(n_i$ infects $n_j) > 0 \iff \tau_i \leq \tau_j$. For a set of cascades $C$ generated from the original $\tau$ infection times, the authors present the likelihood estimation for adjacency matrix A:

% \underbrace{y}_\text{imaginary}
\begin{equation} \label{eq:leskoveclikelihood}
L (A | C) = \prod\limits_{c \in C} \left[ \underbrace{\prod\limits_{i; \tau_{i}^{c} < \infty} (1 -  \prod\limits_{j; \tau_{j}^{c} < \tau_i} (1 -  (\tau_{j} - \tau_i)A_{j,i}) )}_{\text{infected } n_i} \cdot \underbrace{\prod\limits_{i; \tau_{i}^{c} = \infty} \prod\limits_{j; \tau_{j}^{c} < \infty}(1 - A_{j,i})}_{\text{uninfected } n_i} \right]
\end{equation}
%$

Equation \ref{eq:leskoveclikelihood} is straightforward. Over all cascades (outermost product) there are two groups of terms: (infected $n_i$) for each $i$, all node pairs $n_i,n_j \in c$ where $\tau_{i} \leq \tau_{j}$, the innermost product yields the probability of infection time $\tau_{i}$ given $\tau_{j}$, the superscript $c$ is used here, $\tau_{i}^{c}$ to indicate that $n_i$ is infected within `this' cascade, otherwise its infection time is set to $\infty$. The right grouping of products (uninfected $n_i$) calculates the probability that $n_i$ is never infected, given each node $n_j$ adjacent and infected at some finite time in $c$. 

The authors reformulate this likelihood as a convex geometric program to find an optimal $A$ by minimizing the negative log likelihood. This yields the exact solution to the maximum likelihood of the weighted adjacency matrix $A$ under all cascades. The CONNIE model, and most of the subsequent work, is evaluated on synthetic network models, where the underlying network is explicitly known. These methods then also typically present qualitative results on real-world datasets. Below, we will look at related work addressing the limitations of this model and problem formulation: 

%rate of transmission function be a function of time.  
\subsubsection{Submodularity of network inference}
\label{subsubsec:submodularity}

CONNIE uses a geometric program and is not scalable in the number of nodes. Related work \cite{Gomez-Rodriguez:2012:IND:2086737.2086741} (named NETINF) solves a simplified problem in a scalable way by fixing an edge weight probability $\beta$ (\emph{e.g.,} all $A_i,j = \beta$ in the above formulation). For many applications the assumptions of NETINF hold, and scalability is desirable. The main insight of this method is that we can use only the most likely propagation tree on a set of nodes in a cascade $c$. An approximation method can be defined:  

\begin{equation} \label{eq:leskovecexp}
P(C|G) = \prod\limits_{c \in C}~\sum\limits_{T \in T_c(G)}P(c|T) \approx \prod\limits_{c \in C}\smash{\displaystyle\max_{T \in T_c(G)}} P(c|T)
\end{equation}

where $T_c$ defines the set of spanning trees on the nodes in $C$ and the maximum spanning tree is found using edge weights inversely proportional to the difference in infection times, $\Delta_{j,i} = \tau_i - \tau_j$. This likelihood is marginalized on the addition of edges, and the improvement in log-likelihood is proved to be monotonic and submodular, so edges can be greedily selected with an approximation factor of $(1 - 1/e)$ \cite{Nemhauser1978}.

\subsubsection{Inferring rates of transmission}
\label{subsubsec:rates}

The transmission model of \cite{Myers2010} assumes repeated Bernoulli trials of fixed probability. In many applications, susceptibility may vary with time. \cite{ICML2011Gomez_354} (named NETRATE) introduces transmission likelihood functions which vary over time. The method infers a matrix of maximum likelihood transmission rates, according to the input infection times. NETRATE assumes a susceptible-infected infection model. For an infected node $n_j$ and uninfected node $n_i$, and an arbitrary time-step $\tau_*$, $\tau_j \leq \tau_* \leq \tau_i $, the authors define a conditional transmission likelihood function $f$, a survival likelihood $S$, and an instantaneous hazard function $H$: 

\begin{equation} \label{eq:f_transmission}
	f(\tau_*|\tau_j, \alpha_{j,i}) =
	 \begin{cases}
	  \alpha_{j,i} \cdot e^{-\alpha_{j,i}(\tau_* - \tau_j)} & \text{if } \tau_j < \tau_*\\
	  0       & \text{otherwise} 
	 \end{cases}
\end{equation}

\begin{equation} \label{eq:S_survival}
S(\tau_*|\tau_j, \alpha_{j,i}) = 1 - F(\tau_*|\tau_j, \alpha_{j,i})
\end{equation}

\begin{equation} \label{eq:H_hazard}
H(\tau_*|\tau_j, \alpha_{j,i}) = \frac{f(\tau_*|\tau_j, \alpha_{j,i})}{S(\tau_*|\tau_j, \alpha_{j,i})}
\end{equation}

$f(\tau_*|\tau_j, \alpha_{j,i})$ defines the conditional transmission likelihood function: given $n_j$ is infected at time $\tau_j$ and directed edge $\langle n_j, n_i \rangle$ has transmission rate $\alpha_{j,i}$, Equation \ref{eq:f_transmission}  is a form of this likelihood, using an exponential model. The authors also propose a Power Law, and a Rayleigh form which are excluded for brevity. Equation \ref{eq:S_survival} defines $S$ the survival function of $n_i$, using the cumulative density of $f$, and Equation $\label{eq:H_hazard}$ defines the instantaneous infection rate for time $t_*$. 

Each transmission likelihood model, takes as input $\alpha_{i,j}$, and the infection times $\tau_i$, $\tau_j$. The task is to adjust each $\alpha_{i,j}$ to learn the maximum likelihood for the matrix of transmission rates $A= \alpha_{j, i}, (i,j) \in \{1...N\}^2, j\neq i$, optimizing for all cascades. Very similar to the optimization used in CONNIE, the authors use a negative log likelihood which is provably convex, under the constraints $\alpha_j,i \geq 0$.

\begin{figure}[h]
\centering{\includegraphics[width=0.75\columnwidth]{figs/diffusion_fit}}
\caption{From \cite{NIPS2012_4582}, demonstrating poor fit of parametric models to observed transmission data.}
\label{fig:diffusion_fit}
\end{figure}

\subsubsection{Inferring heterogeneous influences}
\label{subsubsec:heterogeneous}

One important limitation of the NETRATE method is that the transmission models must be of an explicit form, parameterized by the transmission rate $\alpha_{i,j}$, and $\Delta_{j,i}$. However, Figure \ref{fig:diffusion_fit} shows real transmission data between blog sites in the MemeTracker\footnote{http://www.memetracker.org/} dataset, where transmission data has a multimodal distribution over time and poorly fits the Exponential or Rayleigh transmission models. This multimodality agrees with intuition because a user's attention may be periodic and discontinuous on blogs, social networks, and face-to-face interactions. For example, assuming typical work hours, the likelihood of the blog entry appearing at midnight may be less than the likelihood for the next morning, yielding this multimodal distribution of transmission events.

\cite{NIPS2012_4582} (named KernelCascade) extends NETRATE, addressing this limitation. The key addition of this work is to kernelize the hazard function $H(\tau_*|\tau_j, \alpha_{j,i})$ over $m$ kernels. Similar to the NETRATE method, the authors use a kernel density function $g(\bullet)$ to kernelize the survival function $S(\tau_*|\tau_j, \alpha_{j,i})$.

\begin{equation} \label{eq:kernel_hazard}
H(\tau_i|\tau_j, \alpha_{j,i}) = \sum\limits_{l=1}^m \alpha_{j,i}^l k(\tau_l, \Delta_{j,i})
\end{equation}

Equation \ref{eq:kernel_hazard} defines $m$ kernels on the distribution of differences in time between an $n_i, n_j$: $\Delta_{j,i} = \tau_i - \tau_j$, where the rate matrix $A= \alpha_{j,i}$ now becomes a three-dimensional coefficient space where each $\boldsymbol\alpha_{j,i}$ is now a vector of length $m$\footnote{Bold indicates vectorized methods and variables}. The authors use a Gaussian radial basis function (RBF) although any kernel with a closed-form integral will be suitable. KernelCascade seems to introduce further parameter sensitivity because the RDF kernel accepts a bandwidth parameter $\sigma$, over a user-specified $m$ number of kernels. However this is inconsequential because larger $m$ only allows for better approximation of the transmission rate probability density, under more narrow $\sigma$, at a greater number of coefficients to represent the kernel. The authors define the kernel density function in the straightforward way for the $l$-th kernel:

\begin{equation} \label{eq:kernel_density}
g_l(\Delta_j,i) = \int\limits_{0}^{\Delta_{j,i}} k(\tau_l, x)dx
\end{equation}

Then, we can rewrite the kernelized likelihood function over all $\mathbf{\alpha_{j,i}}$ given a set of cascades $C$,  over the $m$ kernels:

\begin{equation} \label{eq:kernel_full_likelihood}
L(\mathbf{A}|C) = - \sum\limits_{i}^N \left( \sum\limits_{j \neq i}^N~~\underbrace{\sum_{c \in C; \tau_j^c < \tau_i^c} \boldsymbol\alpha_{j,i}\mathbf{g}(\Delta_{j,i})}_{\text{uninfected } n_i} + \underbrace{\sum\limits_{c \in C; \tau_i \leq T^c} log \sum\limits_{\tau_j^c< \tau_i^c} \boldsymbol\alpha_{j,i}\mathbf{k}(\Delta_{j,i})}_{\text{infected } n_i} \right)
\end{equation}

Similar to that of NETRATE, Equation \ref{eq:kernel_full_likelihood} is the minimum log likelihood formulation, varying $\mathbf{A} = \boldsymbol\alpha_{j,i}$. The left bracketed sum uses the kernel density function $\mathbf{g}(\Delta_j,i)$ to calculate the likelihood of survival on the coefficient vector $\boldsymbol\alpha_{j,i}$ over all $j$. The right bracketed sums calculate the likelihood of infection using the kernelized instantaneous hazard function on the duration $\Delta_{j,i}$. 

\subsubsection{Lower bounds on cascade complexity}
\label{subsubsec:abrahao}
While subsequent methods such as NETRATE and KernalCascade have focused on developing more robust and flexible models, several studies have provided approximation guarantees on simpler models, and give near-exact algorithms for network construction given a large number of traces. Cascade complexity describes the number and/or length of cascades which are necessary to reconstruct a network with high probability. \cite{Abrahao:2013:TCN:2487575.2487664} propose an efficient algorithm for trees and bounded-degree graphs, using $O(\text{ log } n)$ and $O(n\text{ log }n \cdot poly(d_{max}))$ cascades, respectively, where $d_{max}$ is the maximum degree in the graph. For a degree-bounded graph, the proposed solution uses is a simple subset scoring method which builds a likely neighborhood for each $n_i$, over all traces. The algorithm is also able to construct networks only using the \emph{first} edge in each trace as input. The authors show that on the four datasets tested, the first edge approximation performs somewhat competitively against the NETINF method, and surpasses it even on a modest number of input cascades. This suggests that the added information from longer cascades is relatively less than the first edge, and has very practical implications on datasets such as Twitter where real cascades in the form of retweets may be very short.

Similar to the above work, \cite{Netrapalli:2012:LGE:2318857.2254783} develop (1) a greedy approach on trees, for constructing the true neighborhood of $n_i$, $N(i)$ with high probability, using $O(d_i \text{ log } n)$ cascades where $d_i$ is the degree of $n_i$ (or $O(d_{max} \cdot n \text{ log } n)$ for the entire tree), and (2) an MLE method on arbitrary graphs for the same task, using $O(d_i^2\text{ log } n)$ cascades, (or $O(d_{max}^2 \cdot n\text{ log }n)$ for the entire graph). The method is evaluated on a Twitter follower-following directed graph, with simulated cascades using the independent cascade model. Note that these bounds are very similar to those developed by \cite{Abrahao:2013:TCN:2487575.2487664}.

\subsubsection{Limitations and open problems}
This area of research has grown considerably because of the availability of accurate cascade data from blogs and social network sites. However, in many applications it may be easier to observe potential interactions (see: Figure \ref{fig:model}), and the transmitted information may be hidden. For example, on a set of possible interactions, we want to discover \emph{which} interactions between \emph{whom} propagated information which best explains some repeated action (\emph{e.g.,} collective decision-making). Applying information flow analysis on these interaction data (see Section: \ref{subsec:interaction}) may be very useful to infer networks consistent with labeled event data. 

The sensitivity of latent network construction using cascades with infection-time uncertainty is unexplored. While blog entries and other online information networks are associated with exact timestamps, many other applications may have significant uncertainty in the timestamp of infection, such as epidemiology where the exact time of individual infection may be approximated by hours or days. The space of realizable networks using these methods may be very large even under modest uncertainty envelopes, and the growth of cascade complexity vs. uncertainty models (see: \ref{subsubsec:abrahao}) is also unknown. 




==> work-known-networks.tex <==
\subsection{Stand-alone network construction} \label{subsec:known}
 
The stand-alone network construction pattern seeks to construct a network which best represents known relations between the entities in the non-relational input dataset. This is done for at least two reasons: first, the learned edge definition can be informative or explanatory to the nature of the relations, and second, the constructed network can be used for knowledge discovery, finding unknown or anomalous relations between entities which can be directly tested according to the application.

\begin{figure}
\centering{\includegraphics[width=0.75\columnwidth]{figs/dream5}}
\caption{From \cite{Marbach2012}, describing the experimental design of the DREAM5 network inference challenge.}
\label{fig:dream5}
\end{figure}

Gene regulatory networks are a well-studied instance of this network construction pipeline. Gene regulation refers to the direct or indirect interaction of genes in the cell, typically measured by expression profiles under differing experiments or time trials. Figure \ref{fig:dream5} illustrates an ensemble method for gene regulation. The authors (1) generate a ground truth network on three species using experimental trials as well as synthetic network data. In (2), these experiments yield four different datasets of biologically-tested networks of gene regulation, as well as the raw (non-relational) gene expression. A set of 29 methods produce (3) network inference results on each of the four datasets. These methods use a broad range of strategies: regression, mutual information, correlation, bayesian networks, ``other'' methods (e.g. random forests, neural networks, gaussian mixture models, etc.) and combined methods (e.g. rank average across multiple measures). This list demonstrates the maturity and variety of methods applied to this problem. These method use pairwise (e.g. gene-to-gene correlation) or group-wise (e.g. many-to-one group LASSO) measures of interaction intensity, which yield a directed, unweighted network signifying ``gene A regulates gene B''. The authors (4) integrate these 29 different inferred networks to produce an ensemble network. This network is (5) validated against the ground-truth networks generated in step (1). Finally, the authors show that the ensemble method discovered $59$ potential interactions, of which $29$ show some support, and $20$ show strong support for being biologically significant.     

We will look at several example GRN inference methods.\footnote{to do.}  

%build a network representation from data without an explicit relational structure (e.g. gene expression trials) and

% be studied for potentially unknown relations.    The problem of network construction in the context of Gene Regulatory Networks (GRNs) is to 


%\cite{Marbach2012}  \cite{22824380} \todo{tie Clark et al to cascades using ERGM}

==> work-prediction.tex <==


% 
% no objective function
% can all local, mesoscopic, and global objectives be constructed at the same time?  
